Tubular Shape Aware Data Generation for Semantic Segmentation in Medical Imaging

Chest X-ray is one of the most widespread examinations of the human body. In interventional radiology, its use is frequently associated with the need to visualize various tube-like objects, such as puncture needles, guiding sheaths, wires, and catheters. Detection and precise localization of these tube-like objects in the X-ray images is, therefore, of utmost value, catalyzing the development of accurate target-specific segmentation algorithms. Similar to the other medical imaging tasks, the manual pixel-wise annotation of the tubes is a resource-consuming process. In this work, we aim to alleviate the lack of the annotated images by using artificial data. Specifically, we present an approach for synthetic data generation of the tube-shaped objects, with a generative adversarial network being regularized with a prior-shape constraint. Our method eliminates the need for paired image--mask data and requires only a weakly-labeled dataset (10--20 images) to reach the accuracy of the fully-supervised models. We report the applicability of the approach for the task of segmenting tubes and catheters in the X-ray images, whereas the results should also hold for the other imaging modalities.

==> tables/siraz.t1.tex <==
\begin{table*}[ht]
\caption{Comparison of models trained on Manual (Smoothed mask, Hand-drawn) and Generated (GAN-drawn) synthetic data. ``Sm. mask'' corresponds to smoothed mask. ``S.T.'' indicates whether the dataset was adapted using a style transfer. Bold font shows statistically significant best result. BCE corresponds to basic binary cross-entropy loss.}
\begin{center}
	\begin{tabular}{c|ccccc||ccccc}
		                       \textbf{Method} & \textbf{SoftDice}     & \textbf{Dice}         & \textbf{Precision}    & \textbf{Recall}       & \textbf{Hausdorf} & \textbf{SoftDice}     & \textbf{Dice}         & \textbf{Precision}    & \textbf{Recall}       & \textbf{Hausdorf}     \\
		\hline
		& \multicolumn{5}{c}{\textit{Loss: BCE,w=1}} & \multicolumn{5}{c}{\textit{Loss: BCE,w=8}} \\
		\hline
		 Sm. mask        & 6.8$\pm$2.4           & 6.0$\pm$2.1           & 51.4$\pm$5.1          & 3.4$\pm$1.4           & 8.28$\pm$0.06          & 11.0$\pm$0.6          & 10.7$\pm$0.6          & 49.6$\pm$1.6          & 6.6$\pm$0.5           & 8.20$\pm$0.05          \\
		 
		                                    Sm. mask+S.T.        & 14.3$\pm$1.7 &	13.2$\pm$1.9 &	68.5$\pm$1.7 &	7.9$\pm$1.4	& 8.15$\pm$0.07           & 22.9$\pm$2.5 &	24.3$\pm$3.2 &	60.2$\pm$1.5 &	17.3$\pm$2.7 &	8.34$\pm$0.054 \\
		                                    Hand-drawn        & 40.0$\pm$0.9          & 42.2$\pm$1.1          & 81.5$\pm$1.2 & 31.2$\pm$1.0          & 7.14$\pm$0.21          & 44.9$\pm$0.6 & 51.7$\pm$1.1          & \textbf{62.3$\pm$1.1} & 51.7$\pm$3.0          & \textbf{7.23$\pm$0.29} \\
		                                    Hand-drawn+S.T.        & 40.4$\pm$0.4 &	44.1$\pm$0.5 & 80.5$\pm$0.6 & 32.9$\pm$0.4 & 7.18$\pm$0.05  & 44.4$\pm$1.1 & 53.8$\pm$0.5 & 55.5$\pm$2.0 &	59.6$\pm$0.9 & 7.54$\pm$0.14 \\
		                                    Ours GAN           & \textbf{41.7$\pm$0.9} & \textbf{46.0$\pm$0.8} & 78.0$\pm$1.2          & \textbf{35.6$\pm$0.7} & \textbf{7.11$\pm$0.04}   & 41.7$\pm$1.9          & 51.8$\pm$2.0          & 51.4$\pm$2.1          & \textbf{60.8$\pm$1.1} & 7.9$\pm$1.0            \\
		\hline
				& \multicolumn{5}{c}{\textit{Loss: BCE + Dice}} & \multicolumn{5}{c}{\textit{Loss: clDice}} \\
		\hline
		Sm. mask        & 6.9$\pm$1.5           & 6.7$\pm$1.5           & 47.6$\pm$4.0          & 3.9$\pm$1.0           & 8.28$\pm$0.6  & 6.2$\pm$1.5           & 6.2$\pm$1.5           & 43.1$\pm$4.8          & 3.7$\pm$1.0           & 8.32$\pm$0.07.         \\
		                                    Sm. mask+S.T.        & 15.7$\pm$2.7 & 15.5$\pm$2.8 & 67.3$\pm$2.1 &	9.6$\pm$2.0 & 8.09$\pm$0.7 & 18.6$\pm$2.0 &	18.6$\pm$2.0 &	63.6$\pm$2.2 & 12.1$\pm$1.5 & 8.07$\pm$0.05 \\
		                                    Hand-drawn        & 46.0$\pm$1.6          & 47.1$\pm$1.5          & 76.2$\pm$2.5 & 38.1$\pm$1.0          & 7.02$\pm$0.13 & 44.7$\pm$3.6          & 44.7$\pm$3.6          & 72.6$\pm$3.6 & 35.7$\pm$3.7          & 7.06$\pm$0.13          \\
		                                    Hand-drawn+S.T.        & 50.4$\pm$1.1 &	51.8$\pm$1.4 &	74.8$\pm$2.5 &	43.5$\pm$2.6 &	7.01$\pm$0.03 & 52.1$\pm$0.8 &	52.2$\pm$0.9 &	72.0$\pm$0.5 &	44.8$\pm$1.1 &	7.04$\pm$0.6
 \\
		                                    Ours GAN           & 51.2$\pm$0.9 & \textbf{53.8$\pm$0.7} & 67.4$\pm$1.1          & \textbf{49.6$\pm$1.1} & 7.07$\pm$0.23          & 52.8$\pm$0.6 & 52.8$\pm$0.7 & 67.6$\pm$1.0          & \textbf{47.7$\pm$0.9} & 7.21$\pm$0.46
	\end{tabular}
\end{center}
\label{tab:man_gan}
\end{table*}

==> tables/siraz.t2.tex <==
\begin{table*}[h]
\caption{Tuning models on small amount of labelled data. ``\emph{De novo}'' corresponds to initialization from scratch (with a model pre-trained on ImageNet),``Sm. mask'' corresponds to smoothed mask, ``S.T.'' corresponds to additional style transfer processing, ``GAN'' corresponds to the best validation parameters on the GAN-drawn synthetic data. Bold font emphasizes statistically significant best result.}
\begin{center}
  \begin{tabular}{c|ccccc||ccccc}
     \textbf{Init.} & \textbf{SoftDice}     & \textbf{Dice}         & \textbf{Precision}    & \textbf{Recall}       & \textbf{Hausdorf} & \textbf{SoftDice}     & \textbf{Dice}         & \textbf{Precision}    & \textbf{Recall}       & \textbf{Hausdorf}     \\
    \hline 
     & \multicolumn{5}{c}{\textit{Loss: BCE,w=1, tune using 10 images}} & \multicolumn{5}{c}{\textit{Loss: BCE,w=1, tune using 20 images}} \\
    \hline
     \emph{De novo}         & 31.0$\pm$3.3          & 48.4$\pm$1.7          & 61.5$\pm$2.8          & 44.0$\pm$1.2          & 7.42$\pm$0.14          & 31.4$\pm$5.6          & 51.8$\pm$1.7          & 68.2$\pm$2.7          & 45.2$\pm$2.2          & 7.21$\pm$0.12          \\
                                     Sm. mask          & 53.$\pm$0.4          & 55.6$\pm$0.2          & 68.9$\pm$0.5          & 50.4$\pm$0.0          & 6.90$\pm$0.02 & 54.0$\pm$0.4          & 57.0$\pm$0.4          & 74.7$\pm$0.9          & 50.1$\pm$0.4          & 6.76$\pm$0.26          \\
                                     Sm. mask+S.T.          & 54.1$\pm$0.4 &	56.2$\pm$0.4 & 73.7$\pm$0.6 & 49.2$\pm$0.6 & 6.81$\pm$0.04 & 56.2$\pm$0.4 &	58.9$\pm$0.5 &	76.7$\pm$1.1 &	51.6$\pm$1.1 &	6.69$\pm$0.03 \\
                                     Hand-drawn          & 59.2$\pm$0.2          & 62.4$\pm$0.1          & 74.0$\pm$0.4          & 58.1$\pm$0.2          & 6.58$\pm$0.01 & 60.1$\pm$0.0          & 64.0$\pm$0.0          & 77.7$\pm$0.2          & 57.9$\pm$0.1          & 6.46$\pm$0.0           \\
                                     Hand-drawn + S.T. & 59.0$\pm$0.5 & 61.0$\pm$0.5 &	71.7$\pm$0.6 &	57.6$\pm$0.2 &	6.55$\pm$0.02 & 61.3$\pm$0.2 & 63.7$\pm$0.4 &	\textbf{79.0$\pm$0.5} &	56.9$\pm$0.2 &	6.49$\pm$0.07 \\
                                     Ours GAN             & \textbf{61.0$\pm$0.0} & \textbf{63.9$\pm$0.1} & \textbf{75.2$\pm$0.5} & \textbf{59.5$\pm$0.4} & \textbf{6.48$\pm$0.02} & 60.9$\pm$0.5          & 64.6$\pm$0.6          & 78.3$\pm$0.1 & \textbf{58.6$\pm$0.7}          & 6.45$\pm$0.02          \\
    \hline
         & \multicolumn{5}{c}{\textit{Loss: clDice, tune using 10 images}} & \multicolumn{5}{c}{\textit{Loss: clDice, tune using 20 images}} \\
    \hline
     \emph{De novo}         & 49.1$\pm$0.6          & 51.9$\pm$0.4          & 63.4$\pm$1.7          & 48.2$\pm$1.5          & 7.32$\pm$0.07 & 53.8$\pm$0.7          & 56.2$\pm$0.9          & 71.3$\pm$0.4          & 50.1$\pm$1.1          & 6.94$\pm$0.03          \\
                                    Sm. mask          & 55.7$\pm$1.1          & 55.9$\pm$1.1          & 70.5$\pm$0.7 & 49.9$\pm$2.0          & 6.93$\pm$0.06 & 57.5$\pm$0.5          & 57.6$\pm$0.5          & 72.3$\pm$1.0 & 52.2$\pm$1.0          & 6.77$\pm$0.06 \\
                                    Sm. mask+S.T.         & 57.1$\pm$0.1 & 57.3$\pm$0.1 & 72.7$\pm$0.2 & 51.2$\pm$0.1 & 6.81$\pm$0.05 & 58.4$\pm$0.2 & 58.6$\pm$0.2 & 75.5$\pm$0.9 & 51.8$\pm$0.2 & 6.73$\pm$0.04 \\
                                    Hand-drawn          & 61.8$\pm$0.1          & 62.4$\pm$0.1          & 74.5$\pm$0.9          & 57.7$\pm$0.5          & 6.6$\pm$0.0 & 63.2$\pm$0.2          & 63.9$\pm$0.2          & 76.3$\pm$0.2          & 58.8$\pm$0.4          & 6.51$\pm$0.03 \\
                                    Hand-drawn+S.T.          & 61.4$\pm$0.6 &	61.6$\pm$0.6 &	73.7$\pm$1.5 &	56.9$\pm$0.7 &	6.59$\pm$0.03 & 62.5$\pm$0.6 &	62.7$\pm$0.6 &	\textbf{77.5$\pm$0.2} &	56.6$\pm$1.0 &	6.53$\pm$0.07 \\
                                    Ours GAN             & \textbf{64.1$\pm$0.2} & \textbf{64.3$\pm$0.2} & 74.4$\pm$0.1          & \textbf{60.9$\pm$0.4} & \textbf{6.49$\pm$0.02} & \textbf{65.3$\pm$0.1} & \textbf{65.6$\pm$0.2} & 75.6$\pm$0.5          & \textbf{61.9$\pm$0.4}          & \textbf{6.46$\pm$0.1}
  \end{tabular}
\end{center}
\label{tab:tune}
\end{table*}

==> tables/siraz.t3.tex <==
\begin{table*}[h]
\caption{Comparison of modifications for synthetic data generation, ``Intensity'' corresponds to the mean color response regularization, ``Frangi'' to the pipeline of Fig. \ref{fig:diag_synth}, ``Frangi + Cycle'' to  Fig. \ref{fig:diag_synth} augmented with an additional generator for the cycle-consistency.} 
\begin{center}
  \begin{tabular}{c|ccccc||ccccc}
    \textbf{Method} & \textbf{SoftDice}     & \textbf{Dice}         & \textbf{Precision}    & \textbf{Recall}       & \textbf{Hausdorf} & \textbf{SoftDice}     & \textbf{Dice}         & \textbf{Precision}    & \textbf{Recall}       & \textbf{Hausdorf} \\
    \hline
		& \multicolumn{5}{c}{\textit{Loss: BCE,w=1}} & \multicolumn{5}{c}{\textit{Loss: BCE,w=8}} \\
	\hline
   Intensity        & 27.0$\pm$4.3          & 27.1$\pm$4.7          & 74.7$\pm$4.1          & 18.2$\pm$3.6          & 7.72$\pm$0.24     & 38.7$\pm$3.3          & 42.4$\pm$3.8          & \textbf{65.6$\pm$3.2} & 35.8$\pm$3.6          & 8.08$\pm$0.54     \\
                                 Frangi + Cycle & 34.6$\pm$3.6          & 36.5$\pm$4.5          & 75.0$\pm$2.0          & 26.7$\pm$4.2          & 7.43$\pm$0.32     & \textbf{42.3$\pm$1.2} & 48.8$\pm$1.9          & 59.5$\pm$1.2          & 47.2$\pm$3.5          & 7.52$\pm$0.2      \\
                                 Frangi (Ours)        & \textbf{41.7$\pm$1.9} & \textbf{46.0$\pm$2.6} & \textbf{78.0$\pm$2.2} & \textbf{35.6$\pm$2.7} & 7.11$\pm$0.13     & 41.7$\pm$1.9          & \textbf{51.8$\pm$2.0} & 51.4$\pm$2.1          & \textbf{60.8$\pm$1.5} & 7.9$\pm$1.0       \\
                                 
    \hline
		& \multicolumn{5}{c}{\textit{Loss: BCE + Dice}} & \multicolumn{5}{c}{\textit{Loss: clDice}} \\
	\hline
    
    
    Intensity        & 34.1$\pm$3.0          & 34.3$\pm$3.2          & \textbf{76.3$\pm$1.6} & 24.6$\pm$3.1          & 7.69$\pm$0.28 & 31.0$\pm$4.2          & 31.0$\pm$4.2          & 70.8$\pm$2.8          & 21.6$\pm$3.5          & 7.87$\pm$0.18     \\
                                 Frangi + Cycle & 41.0$\pm$1.9          & 42.0$\pm$2.0          & 69.3$\pm$2.1          & 33.7$\pm$2.1          & 7.39$\pm$0.14 & 43.2$\pm$3.6          & 43.2$\pm$3.6          & 70.2$\pm$2.0          & 34.3$\pm$3.8          & 7.42$\pm$0.14     \\
                                 Frangi (Ours)         & \textbf{51.2$\pm$2.4} & \textbf{53.8$\pm$2.5} & 67.4$\pm$1.1          & \textbf{49.6$\pm$3.6} & 7.07$\pm$0.23 & \textbf{52.8$\pm$0.6} & \textbf{52.8$\pm$0.7} & 67.6$\pm$1.0          & \textbf{47.7$\pm$0.9} & 7.21$\pm$0.46
  \end{tabular}
\end{center}
\label{tab:ablation}
\end{table*}

==> tables/siraz.t4.tex <==
\begin{table}[h]
  \caption{Comparison of segmentation models trained on the real data. Evaluation was performed on the out-of-fold predictions.}
  \begin{center}
    \begin{tabular}{c|c|ccccc}
      \textbf{Loss}   & \textbf{SoftDice} & \textbf{Dice} & \textbf{Precision} & \textbf{Recall} & \textbf{Hausdorf} \\
      \hline
        \textbf{BCE,1}  & 59.8$\pm$2.2 & 68.3$\pm$2.7 & 79.4$\pm$1.7 & 62.9$\pm$3.1 & 6.29$\pm$0.65 \\
        \hline
        \textbf{BCE,8}  & 55.8$\pm$3.2 & 63.5$\pm$2.7 & 56.2$\pm$4.2 & 78.4$\pm$2.5 & 7.45$\pm$1.19 \\
        \hline
        \textbf{clDice} & 70.0$\pm$2.0 & 70.2$\pm$2.0 & 74.3$\pm$3.1 & 69.7$\pm$2.4 & 6.38$\pm$5.51 
    \end{tabular}
  \end{center}
  \label{tab:gt}
\end{table}
